Strategies for Arabic Readability Modeling

Automatic readability assessment is relevant to building NLP applications for education, content analysis, and accessibility. However, Arabic readability assessment is a challenging task due to Arabic's morphological richness and limited readability resources. In this paper, we present a set of experimental results on Arabic readability assessment using a diverse range of approaches, from rule-based methods to Arabic pretrained language models. We report our results on a newly created corpus at different textual granularity levels (words and sentence fragments). Our results show that combining different techniques yields the best results, achieving an overall macro F1 score of 86.7 at the word level and 87.9 at the fragment level on a blind test set. We make our code, data, and pretrained models publicly available.

==> TRASH/methods.tex <==
\section{Methods}
\label{methods}
We frame readability assessment as a sequence-level estimation task to classify a given fragment of text as having a readability level of 5, 4 or 3. Using the SAMER Corpus 
dataset annotations on fragment and word levels discussed above, we divide our process in two phases: \textbf{word-level readability tagging}, and \textbf{fragment-level readability tagging}. 
%For the final phase, we attempt both deriving fragment labels from an aggregation of word labels obtained in the first phase, or obtaining them from a fragment-level BERT representation.

\subsection{Word-Level Readability Tagging}
\label{sec:word-level-ragg}
We explore several modeling approaches spanning rule-based to PLMs based models.
% Inspired by previous work on readability assessment, we explore several modeling approaches spanning rule-based to PLMs based models.
In total, we investigate four techniques to tag words according to their readability levels: Maximum Likelihood Estimation (MLE), Lexicon lookup, Frequency tagging, and BERT-based token classification. Each technique uses different sources of complementary data as summarized in 
Table~\ref{tab:approaches}. Moreover, each technique has a different set of parameters, which were tuned to optimize the performance on the development set.

We further investigate combining the systems in a cascaded setup, leveraging their complementary strengths to address the limitations of each system individually.


% After each technique was individually tuned, a system selection approach was followed in which different combinations of Starting and Final Decisions the techniques were applied hierarchically in order to select the most performing setup for the task.

\begin{figure}[t!]
    \centering
    %\includegraphics[width = \columnwidth]{assets/table5.pdf}
    \setlength{\tabcolsep}{1pt}
    %\small
    \begin{tabular}{lcccc}\toprule
&\multicolumn{4}{c}{\textbf{Data Used}} \\\cmidrule{2-5}
\textbf{Tagging} &\textbf{SAMER}  &\textbf{CAMeL} &\textbf{Arabic}  &\textbf{SAMER}  \\ 
\textbf{Method} &\textbf{Corpus}& \textbf{BERT} & \textbf{Treebank} & \textbf{Lexicon }\\\midrule

Lexicon & &X &X &X \\
BERT &X &X & & \\
Frequency &X &Counts & & \\
MLE &X & & & \\
Default L3 & & & & \\
\bottomrule
\end{tabular}
    
    \captionof{table}{Data used in each of the word-level models.}
    \label{tab:approaches}
\end{figure}

% \subsubsection{Starting Decisions}
\subsubsection{Maximum Likelihood Estimation} 
The \textbf{MLE} model constitutes a simple lookup table of the types (i.e., unique words) and their readability levels over the training data. During inference, we pick the readability level of the word that occurred the most in the training data. Evidently, this technique will not generalize to words that do not exist in the training data.
% Our first technique was to count the number of occurrences tagged at each level for each of the types present in the corpus. We tag each type with the level it occurs the most at. On this technique, readability inference is done by search, with the possibility that we are not able to resolve the level of a word.

\begin{figure}[t!]
    \centering
    %\includegraphics[width = 0.9\columnwidth]{assets/table4.pdf}
    %
 %   \small
\begin{tabular}{lrrrr}\toprule
\textbf{All Types} &\textbf{31,940} & & \\\midrule
Level 3 only &22,260 &69.7\% &\multirow{3}{*}{97.2\%} \\
Level 4 only &5,423 &17.0\% & \\
Level 5 only &3,376 &10.6\% & \\\midrule
Levels 4 and 3 &473 &1.5\% &\multirow{4}{*}{2.8\%} \\
Levels 5 and 3 &253 &0.8\% & \\
Levels 5 and 4 &89 &0.3\% & \\
Levels 3, 4, and 5 &66 &0.2\% & \\
\bottomrule
\end{tabular}
    
    \captionof{table}{Types and their readability levels according to the MLE model in the Dev set.}
    \label{tab:types}
\end{figure}

Table~\ref{tab:types} presents statistics of applying the MLE approach on the Dev set. The statistics show that in a number of cases, the same word could be assigned to more than one readability level. This highlights the need to model the full fragment context to resolve ambiguity. 

\subsubsection{Lexicon} 
Our second model, \textbf{Lex},  leverages the SAMER Readability Lexicon \citep{al_khalil_large-scale_2020}. The lexicon consists of 40K lemmas that were manually annotated with their readability levels starting from Level 1 to Level 5. For the purposes of our task, we consider words of levels 1 and 2 to be included under Level 3 words. During inference, we use the morphological analyzer and disambiguator built by \newcite{inoue2022morphosyntactic} that is available in CAMel Tools \cite{obeid_camel_2020} to extract the lemma and part-of-speech tag for each word to infer the readability level from the lexicon.
%
Since the disambiguator focuses on morphosyntactic features, it  commonly returns multiple top lemma analyses for the same word. We tiebreak on the lowest readability level first followed by lemma-log probability when selecting the lemma. This choice was determined empirically (see Appendix \ref{app:tiebreak}). 


It is worth noting that the SAMER Readability Lexicon was used in the annotation of the SAMER Corpus, however its use was not prescriptive and annotators were asked to both adjust the suggested levels and perform any insertion, deletion, or replacement decision they saw fit to reduce the readability levels of the parallel documents. This means that, in many cases, the annotations differed from the lexicon suggestions.

%\textcolor{red}{FIX} Similar to our approach, the aid resolved the lemma and level of each word through a disambiguator, and categorized words it was unable to resolve as maximum level \citep{alhafni-etal-2024-samer}. Motivated by the need to examine the discrepancies between automatic lemma-level tagging and human annotation, we use this resource to assess the performance of such resources as the base for unsupervised techniques for word and fragment-wise readability assessment, and to shed light on what the differences between these lemma-based suggestions and the ground truth provided by the annotators is.


\subsubsection{Frequency-Based Word Tagging}
%https://github.com/CAMeL-Lab/Camel_Arabic_Frequency_Lists 

% Inspired by previous work on readability assessment through frequency analysis in large corpora, we explore different approaches to derive readability levels from frequency data.
We explore different approaches to derive readability levels from frequency data.
We leverage our training data and link it with type frequency data derived from a corpus of 12B words (11M types) used to pretrain the CAMeLBERT models \citep{inoue_interplay_2021}.

% Following previous work on readability level assessment by frequency in large corpora, we attempt different approaches to derive readability levels from frequency data based on linking information from our training data to the type frequency data from a corpus of 1B words (11M types) used to train the CAMeLBERT models \citep{inoue_interplay_2021}.

\paragraph{Tagging on Thresholds (Threshold-Freq)} 

We obtain a frequency distribution of token readability levels from our training data (seen in 
Table~\ref{tab:tokens}). Following the intuition that 
%more << This is incorrect... it's less difficult words tend to appear more often
less difficult words tend to appear more often, we sorted the types we obtained from the CAMeLBERT pretraining data by their frequency. We assigned Level 3 to the most frequent types, with Levels 4 and 5 assigned according to the frequency distribution observed in our training data.

\paragraph{Tagging on Bins (Binning-Freq)}
% Following the intuition that similarly leveled types are similarly ranked in frequency, we divided the frequency rankings in equally sized bins based on cumulative frequency. We leverage our type-labeled training data and collect, for every bin, the number of known types and their level. We thus label all the types of the bin with the majority known level within.
% As bins get smaller, there is a lower chance that every bin has known tokens, a case in which we default to one of the three levels. We experiment with different bin sizes and default level options, and select a convenient variation as measured by accuracy and average F\textsubscript{1} score across classes. Further details on these experimental variations are available on Appendix~\ref{app:binning}. We find that dividing the frequency space into 10,000 bins has the highest performance among the variations.

Based on the assumption that types of a certain readability level tend to have similar frequencies in a large corpus, we divide the frequency-sorted types from the CAMeLBERT pretraining data into equally sized bins. Utilizing our training data, we assign a readability level to all the types within each bin according to the majority readability level found in that bin. During inference, if words are not observed in any bin, we default to assigning a readability level of 5, reflecting the expectation that rare words are typically harder to read. We empirically experiment with different number of bins and identify that dividing the sorted-frequency types into 10,000 bins yields the highest performance in terms of accuracy and macro F\textsubscript{1} score. Additional details can be found in Appendix~\ref{app:binning}.





\subsubsection{BERT Token Classification}

We build a word-level classifier by leveraging a Transformer-based pretrained language model. There are many Arabic monolingual
BERT \cite{devlin-etal-2019-bert} models available such as AraBERT \cite{antoun-etal-2020-arabert}, ARBERT \cite{abdul-mageed-etal-2021-arbert}, and JABER \cite{ghaddar-etal-2022-revisiting}. However, we chose to use CAMeLBERT MSA \cite{inoue-etal-2021-interplay} as it was pretrained on the largest MSA dataset to date. We fine-tune CAMeLBERT MSA using Hugging Face’s Transformers \cite{wolf-etal-2020-transformers} by adding a fully-connected linear layer with a softmax on top of its architecture. Given that BERT operates at the subword-level (i.e., wordpieces), we assign to each subword the readability level of the word it belongs to. During inference, we label each word according to the highest readability level among its subwords. We fine-tune our model on a single GPU for 10 epochs with a learning rate of 1e-5, a batch size of 32, and a maximum sequence length of 30.


% This technique leverages the use of BERT for transfer learning of classification tasks, as BERT hidden states have been successfully probed for information on a variety of linguistic features, and, crucially, because BERT outputs for tokens include contextual information, which could be leveraged to solve contextual differences techniques such as MLE are blind towards. In order to leverage BERT for readability leveling, we frame our objective as a token classification task, and take an approach similar to those used for other token classification tasks such as named entity recognition and part-of-speech tagging: we apply a linear layer to each of the representations of the tokens in the sentence in order to have a prediction for each token.
%
% BERT, however, tokenizes fragments of texts into sub words. Given that the data obtained from the corpus is tagged at the word level, we enact two changes in order to enable training and evaluation:
%\begin{itemize}
%    \item 
    % during \textbf{training} we  assign to each subword the label of its containing word;
    %\item 
    % and during \textbf{evaluation}, we assign to a word the highest level among its subwords. 
    %We compute our metrics on these outputs.
%\end{itemize}
%
% We used the CAMeLBERT MSA model \citep{inoue_interplay_2021}. %namely those in Classical Arabic, Modern Standard Arabic, and a mix of the two, following their insights on the effect of dialectal proximity on the performance of downstream tasks. 
%as it performed best on the tuning we conducted 



%\subsubsection{System Combination}
%In addition to evaluating the various systems discussed above, we also consider their combinations to resolve non-final decisions from some systems using other systems applied in layers:
%
%We establish experimental variations in which a Starting Decision (or a layering of both Starting Decisions) is layered on top of a Final Decision. 
%If a word is unable to be resolved by the starting layer, it is deferred to the layer below, until reaching a final decision. These layered experiments aim to establish which final decision methods are more suitable for each of the starting decisions, and which starting decision should be applied first. We evaluate these systems both on word and fragment Leveling accuracy and class-wise F\textsubscript{1} scores.
%
%\textbf{Layered Experiment Tuning.} We are able to modify which types are backed off to the next layers when using the MLE technique as first decision by setting two thresholds to make a decision on a word: minimum confidence level and minimum occurrences seen. We do this with the intention of backing off to the lower layers of of the system instead of using a potentially unreliable MLE estimate. We cross-validate these two parameters on the development set, and choose the variation with the highest performance in word Leveling accuracy and class-wise F\textsubscript{1} scores. We find that a confidence threshold of 0.85 and no minimum occurrence threshold gives us the best results.


\subsubsection{System Combination}
In addition to evaluating the various systems discussed above, we consider their combinations to exploit their complementarities.
%
Our approach to combining the systems runs the Lex and MLE models first (independently and together in different orders -- four combinations) followed by one of the other six models (default level 3, 4, or 5, Binning Frequency, Threshold Frequency, or BERT).  The total is 24 combinations layered in two or three steps. 
See Table~\ref{tab:all-combos} in Appendix~\ref{app:layers}.
%
Since the early layers, Lex and MLE, do not handle unknown words, the later layers resolve the these cases. 
%
We evaluate all these system combinations on both word and fragment leveling in terms of  accuracy and class-wise F\textsubscript{1} scores.

\paragraph{Tuned MLE} 
In addition to the above, we consider a Tuned MLE model variation in the system combination, where we explore different variables for what to consider in-vocabulary MLE words: minimum confidence level and minimum occurrences seen. We empirically determine the best value by cross-validation on the development set and judging by word leveling accuracy and class-wise F\textsubscript{1} scores. We find that a confidence threshold of 0.85 and no minimum occurrence threshold gives us the best results.


\subsection{Fragment-Level Readability Tagging}
We consider two approaches to fragment-level tagging: a direct BERT-based approach and an aggregation of the word-level predictions.


\subsubsection{BERT Fragment Classification}
We train a fragment-level by fine-tuning CAMeLBERT MSA. In a similar approach to the word-level BERT classifier, we add a fully connected linear layer on top of the representation of the whole fragment (i.e., \texttt{[CLS]} token embedding).
% We experiment with different ways of obtaining the fragment representation from the BERT model: using the [CLS] token, and mean and max-pooling, as well as, similarly to the word-level approach, testing the different dialectal variations of the same. Details on these results can be found on Appendix \ref\input. We select mean-pooling on the Modern Standard Arabic version of CAMeLBERT.
We fine tune our model using Hugging Face's Transformers \cite{Wolf:2019:huggingfaces} on a single GPU for 10 epochs with a learning rate of 5e-5, a batch size of 32, and a maximum sequence length of 20.

\subsubsection{Aggregating Word-Level Predictions}
%\textbf{Comparison with Wordwise Systems}
After we obtain the word-level predictions using the systems introduced in \S\ref{sec:word-level-ragg}, we assign to each fragment the highest readability level found among its words. This allows us to compare the performance of aggregated word-level decisions with single fragment-level decisions in terms of readability leveling.


% We aggregate the word-level predictions obtained from the systems developed in the previous section into fragment levels by assigning to each fragment the highest level among its words. This way, we can compare the readability Leveling performance of aggregated word-level decisions against single fragment level decisions.



% We aggregate the word levels obtained from the systems developed in the previous section into fragment levels by assigning to each fragment the highest level among its words. This way, we can compare the readability Leveling performance of aggregated word-level decisions against single fragment level decisions.
